A self-supervised learning strategy for postoperative brain cavity segmentation simulating resections

Accurate segmentation of brain resection cavities (RCs) aids in postoperative analysis and determining follow-up treatment. Convolutional neural networks (CNNs) are the state-of-the-art image segmentation technique, but require large annotated datasets for training. Annotation of 3D medical images is time-consuming, requires highly-trained raters, and may suffer from high inter-rater variability. Self-supervised learning strategies can leverage unlabeled data for training. We developed an algorithm to simulate resections from preoperative magnetic resonance images (MRIs). We performed self-supervised training of a 3D CNN for RC segmentation using our simulation method. We curated EPISURG, a dataset comprising 430 postoperative and 268 preoperative MRIs from 430 refractory epilepsy patients who underwent resective neurosurgery. We fine-tuned our model on three small annotated datasets from different institutions and on the annotated images in EPISURG, comprising 20, 33, 19 and 133 subjects. The model trained on data with simulated resections obtained median (interquartile range) Dice score coefficients (DSCs) of 81.7 (16.4), 82.4 (36.4), 74.9 (24.2) and 80.5 (18.7) for each of the four datasets. After fine-tuning, DSCs were 89.2 (13.3), 84.1 (19.8), 80.2 (20.1) and 85.2 (10.8). For comparison, inter-rater agreement between human annotators from our previous study was 84.0 (9.9). We present a self-supervised learning strategy for 3D CNNs using simulated RCs to accurately segment real RCs on postoperative MRI. Our method generalizes well to data from different institutions, pathologies and modalities. Source code, segmentation models and the EPISURG dataset are available at https://github.com/fepegar/ressegijcars .

==> tex/sections/__latexindent_temp.tex <==
\section{Experiments and results}

\subsection{Data}
\label{sec:data}
\input{tex/sections/experiments_and_results/data}


\subsection{Network architecture and implementation details}
\input{tex/sections/experiments_and_results/implementation}

\subsection{Processing and augmentation during training}
\input{tex/sections/experiments_and_results/processing_training}


% % Specify this for each experiment?
% Training occurred for 60 epochs, and the learning rate was divided by 10 every 20 epochs.
% %
% %and the training set was shuffled at the beginning of each epoch.
% %
% %
% 90\% of the images were used for training and 10\% for validation.

% % Above lines removed to gain some space


\subsection{Experiments}

Bonferroni correction
Type of statistical test


\subsubsection{Self-supervised learning: training with simulated resections only}

% % TODO: VERIFY THAT NOTHING IS MISSING. Move to supplementary

% The following parameters were used to generate simulated resections
% (see \cref{sec:simulation}):
% $f = 16$,                                           % frequency
% $\omega = 4$,                                       % octaves
% $\gamma = 0.5$,                                     % persistence
% $\zeta = 3$,                                        % scaling
% $\bm{\mu} \sim \mathcal{U}(0, 1000)$,               % offset
% $\lambda \sim \mathcal{U}(1, 2)$,                   % radii ratio
% %$r_o = 3$,                                          % ball radius for resectable hemisphere mask
% %${d_m = 4}$,                                        % median filter kernel
% and ${\bm{\sigma}_{\bm{A}} \sim \mathcal{U}(0.5, 1)}$.   % std to blur the mask
% %and $r_e = 1$.                                      % ball radius erosion of ventricles mask
% % TODO: change this
% The ellipsoid volume $v$ is sampled from volumes
% of manually segmented cavities from Rater A (see \cref{sec:data}).

In our first experiment, we assess the relation between the complexity of the resection simulation and the segmentation performance.
We train using simulated data from the publicly available dataset
$D\st{C} = \{ \X_{\text{C}_i} \}_{i = 1}^{n\st{C}}$, where $n\st{C} = 1813$ (\cref{sec:data}).
We use 90\% of the images in $D\st{C}$ for the training set
$D\st{Ctrain} = \{ \X_{\text{C}_i} \}_{i = 1}^{n\st{Ctrain}}$ and 10\% for validation set
$D\st{Cval} = \{ \X_{\text{C}_i} \}_{i = 1}^{n\st{Cval}}$ ($n\st{Ctrain} = 1632$ and $n\st{Cval} = 181$).
The 133 annotated postoperative images in EPISURG are used for evaluation.

Before training, we precompute and cache a validation set
\begin{equation}
    D\st{Rval}
    = \{ T\st{Aug} \circ \phi\st{R} (\X_{\text{C}_i}) \}_{i = 1}^{n\st{Cval}}
    = \{ ( \X_{\text{R}_i}, \Y_{\text{R}_i})          \}_{i = 1}^{n\st{Cval}}
\end{equation}
where $\phi\st{R}$ is the resection simulation described in \cref{sec:simulation} and $T\st{Aug}$ represents the preprocessing and augmentation described in \cref{sec:preprocessing_augmentation}.
Hyperparameters for $\phi\st{R}$ and $T\st{Aug}$ are specified in the supplementary material\textcolor{red}{[TODO]}.

At each training iteration, $b$ images from $D\st{C}$ are loaded, resected, preprocessed and augmented to obtain a mini-batch of $b$ training instances
$\{ ( \X_{\text{R}_i}, \Y_{\text{R}_i}) \}_{i = 1}^{b}$.
Note that the resection simulation is performed on the fly, which allows us to further augment the space of images with simulated resection cavities.

\paragraph{Effect of resection shape}

To investigate the effect of the simulated cavity on the model performance on real data, we modify $\phi\st{R}$ to generate cuboid- or ellipsoid-shaped resections.
The cuboids and ellipsoid meshes are not perturbed using simplex noise, and cuboids are not rotated.


FIGURE

\paragraph{Effect of resection texture}


\begin{table}
    \centering
    \caption{%
        Caption.
    }
    \label{tab:self}
    \begin{tabular}{ccccl}
        \toprule
        \centering \textbf{WM lesion} &
        \centering \textbf{Blood products} &
        \centering \textbf{Cavity shape} &
        \centering \textbf{Augmentation} &
        \textbf{DSC} \tabularnewline
        \midrule
                        No &                      No &                Cuboid &                   Yes &  57.9 (73.1) \\  % 5
                        No &                      No &             Ellipsoid &                   Yes &  79.0 (20.0) \\  % 9
                        No &                      No &                 Noisy &                   Yes &  79.7 (17.9)* \\  % 2 (baseline)
                        No &                      No &                 Noisy &                    No &  00.0 (00.0) \\  %
                        No &                     Yes &                 Noisy &                   Yes &  00.0 (00.0) \\  %
                       Yes &                      No &                 Noisy &                   Yes &  78.2 (20.3) \\  % 16
                       Yes &                     Yes &                 Noisy &                   Yes &  00.0 (00.0) \\  % 18?
        \bottomrule
    \end{tabular}
\end{table}


\subsubsection{Semi-supervised learning: adding pseudolabels from real resections}


\begin{table}
    \centering
    \caption{%
        The dagger $\dagger$ indicates that a random subset of pseudolabels was used.
    }
    \label{tab:self}
    \begin{tabular}{ccl}
        \toprule
        \textbf{Percentile} & \textbf{Pseudolabels} & \textbf{DSC} \\
        \midrule
                          0 &                     0 & 79.7 (17.9)* \\
                         25 &                     0 & 00.0 (00.0)  \\
                         50 &                     0 & 00.0 (00.0)  \\
                         75 &                     0 & 00.0 (00.0)  \\
                        100 &                     0 & 00.0 (00.0)  \\
                66$\dagger$ &                     0 & 00.0 (00.0)  \\  % replace 66 with the best amongst the others
        \bottomrule
    \end{tabular}
\end{table}


\subsubsection{Finetuning on small datasets}

% \begin{table}
%     \centering
%     \caption{%
%         Caption.
%     }
%     \label{tab:shape}
%     \begin{tabular}{l*3c}
%         \toprule
%         \textbf{Dataset}                              & \textbf{London} & \textbf{Milan} \\
%         \midrule
%         \textbf{Unlabeled}                            &               1 &              0 \\
%         \textbf{Unlabeled + labeled}                  &               1 &              0 \\
%         \textbf{Unlabeled + pseudo-labeled}           &               1 &              - \\
%         \textbf{Unlabeled + labeled + pseudo-labeled} &               1 &              - \\
%         \bottomrule
%     \end{tabular}
% \end{table}

\subsection{Evaluation on brain tumor dataset}


\subsection{Code and models availability}

Resector
IJCARS scripts
Resseg
EPISURG


==> tex/sections/experiments_and_results/semi_supervised.tex <==
\subsubsection{Semi-supervised learning: leveraging real unlabeled resections}
\label{sec:results_semi}

\newcommand{\pseudo}{\st{pseudo}}

In this experiment, we assessed the ability of semi-supervised learning to improve the performance of our baseline model.
We first computed the uncertainty $u(f_{\alpha\beta}, \X\post, n\st{unc})$ for
$D\unl$ (\cref{sec:leveraging_semi}),
all unlabeled images in EPISURG,
using the baseline model and the preprocessing and augmentation transforms (\cref{sec:preprocessing_augmentation}).
We generated pseudolabels and estimated uncertainty from $n\st{unc} = 50$ Monte Carlo \ac{tta} iterations (\cref{sec:leveraging_semi}).
To obtain the final dataset $D\pseudo = \{ (\X_{\text{postop}_i}, \wt{\Y}_{\text{cavity}_i}) \}_{i = 1}^{n\pseudo}$, we selected pseudolabels with $u(\X_{\text{postop}_i}, \cdot) < t\st{unc} = 0.2$, resulting in $n\pseudo = 256$.

We used $D\st{pre,train}$ (\cref{sec:self}) in addition to $D\pseudo$ to train a new model $\fp{sim,semi}(\cdot)$, using the same hyperparameters as in the self-supervised setting (\cref{sec:self}).
To ensure that all batches contain real resections, we use $b - b\pseudo$ images from $D\st{pre,train}$ and $b\pseudo$ images from $D\pseudo$ to compose each mini-batch of size $b$.
We chose $b\pseudo = 2$ for our experiments, i.e., 20\% of the images in each mini-batch contain real resection cavities.

Semi-supervised learning improved the performance of the baseline model from 80.5 (18.7) to 81.5 (17.8) ($p = 0.474$).  % Experiment 37

% trim is "left bottom right top"

\newcommand{\uncertainties}[1]{
    \begin{subfigure}{0.25\textwidth}
        \includegraphics[trim=0 680 642 32, clip, width=0.98\linewidth]{#1_uncertainty}
    \end{subfigure}%
    \begin{subfigure}{0.25\textwidth}
        \includegraphics[trim=642 680 0 32, clip, width=0.98\linewidth]{#1_uncertainty}
    \end{subfigure}%
    \begin{subfigure}{0.25\textwidth}
        \includegraphics[trim=0 0 642 714, clip, width=0.98\linewidth]{#1_uncertainty}
    \end{subfigure}%
    \begin{subfigure}{0.25\textwidth}
        \includegraphics[trim=642 0 0 714, clip, width=0.98\linewidth]{#1_uncertainty}
    \end{subfigure}%
}

\newcommand{\uncertaintiescap}[1]{
    \begin{subfigure}{0.25\textwidth}
        \includegraphics[trim=0 680 642 32, clip, width=0.98\linewidth]{#1_uncertainty}
        \caption{\label{fig:uncertainty_mri}}
    \end{subfigure}%
    \begin{subfigure}{0.25\textwidth}
        \includegraphics[trim=642 680 0 32, clip, width=0.98\linewidth]{#1_uncertainty}
        \caption{\label{fig:uncertainty_std}}
    \end{subfigure}%
    \begin{subfigure}{0.25\textwidth}
        \includegraphics[trim=0 0 642 714, clip, width=0.98\linewidth]{#1_uncertainty}
        \caption{\label{fig:uncertainty_mean}}
    \end{subfigure}%
    \begin{subfigure}{0.25\textwidth}
        \includegraphics[trim=642 0 0 714, clip, width=0.98\linewidth]{#1_uncertainty}
        \caption{\label{fig:uncertainty_pseudo}}
    \end{subfigure}%
}

% image - mean - std - pseudolabeled
% sid=0914
% scp -r dgx:/home/fernando/datasets/real/pseudo/image/$sid\* .
% scp -r dgx:/home/fernando/datasets/real/pseudo/label/$sid\* .
% scp -r dgx:/home/fernando/datasets/real/pseudo/aleatoric/std/$sid\* .
% scp -r dgx:/home/fernando/datasets/real/pseudo/aleatoric/mean/$sid\* .


% bien 0499
% regular 0914  # 568
% mal 0796

\begin{figure}
    \centering
    \begin{minipage}{.2\linewidth}
        \begin{subfigure}{0.875\textwidth}
            \includegraphics[width=\linewidth]{qcd}
            \caption{\label{fig:all_uncertainties}}
        \end{subfigure}
    \end{minipage}%
    \begin{minipage}{.8\linewidth}
        \uncertainties{0796}

        \uncertainties{0914}

        \uncertaintiescap{0499}
    \end{minipage}
    \caption{%
        Generating reliable pseudolabels for semi-supervised learning.
        Image-level uncertainty for the 297 unlabeled postoperative images in EPISURG (\subref{fig:all_uncertainties}).
        Unlabeled postoperative \ac{t1} \ac{mri} (\subref{fig:uncertainty_mri}).
        Voxel-wise uncertainty (\subref{fig:uncertainty_std}) estimated as the standard deviation of the probabilities across all Monte Carlo iterations.
        The mean prediction (\subref{fig:uncertainty_mean}) is thresholded at 0.5 to generate the pseudolabel (\subref{fig:uncertainty_pseudo}).
        Image-level uncertainties for the three cases are 0.805 (top), 0.195 (middle) and 0.025 (bottom)
    }
    \label{fig:uncertainties}
\end{figure}

